QuasiSim: Parameterized Quasi-Physical Simulators for Dexterous Manipulations Transfer

We explore the dexterous manipulation transfer problem by designing simulators. The task wishes to transfer human manipulations to dexterous robot hand simulations and is inherently difficult due to its intricate, highly-constrained, and discontinuous dynamics and the need to control a dexterous hand with a DoF to accurately replicate human manipulations. Previous approaches that optimize in high-fidelity black-box simulators or a modified one with relaxed constraints only demonstrate limited capabilities or are restricted by insufficient simulation fidelity. We introduce parameterized quasi-physical simulators and a physics curriculum to overcome these limitations. The key ideas are 1) balancing between fidelity and optimizability of the simulation via a curriculum of parameterized simulators, and 2) solving the problem in each of the simulators from the curriculum, with properties ranging from high task optimizability to high fidelity. We successfully enable a dexterous hand to track complex and diverse manipulations in high-fidelity simulated environments, boosting the success rate by 11\%+ from the best-performed baseline. The project website is available at https://meowuu7.github.io/QuasiSim/.

==> articles/ABLATIONS-copy.tex <==
\section{Ablation Study} \label{sec:ablations}

We conduct a wide range of ablation studies to validate the effectiveness of some of our crucial designs, including the parameterized analytical physics model, the parameterized residual physics, the role of the local force network, the necessity of introducing a physics curriculum into the optimization, and how the design on the curriculum stages affects the result. 



\noindent\textbf{Parameterized analytical model.}
The skeleton of the quasi-physical simulator is an analytical physics model. The intuition is that the parameterized simulator with such physical bias can be optimized towards a realistic simulator more easily than training pure neural networks for approximating. To validate this, we ablate the analytical model and use neural networks to approximate physics in Bullet directly (denoted as ``Ours w/o Analytical Sim.''). The quantitative (Table~\ref{tb_exp_ablations}) and qualitative (Fig.~\ref{fig_abl_stapler}) results indicate that the physical biases brought by the analytical model could help the parametric simulator to learn better physics in the contact-rich scenario. For instance, in the example demonstrated in Fig.~\ref{fig_abl_stapler}， the ablated version fails to guide the robot hand to successfully pinch the object in the second figure. 
% optimizing the parameterized sim
% which severs as an analytical bias for the simula
% The intuition is that optimizing 
% The model outlines the simulations 
% The model outlines the simulations
% The model outlines the simulations such as the contact region identification and the contact force model. The intuition is that the analytical model gives strong physical biases for the parametric simulator. Therefore optimizing it to approximate a more realistic simulator would become easier than training neural networks to approximate the physics. To validate this, we ablate the analytical model and use neural networks to approximate physics in Bullet directly (denoted as ``Ours w/o Analytical Sim.''). The quantitative (Table~\ref{tb_exp_ablations}) and qualitative (Fig.~\ref{fig_abl_stapler}) results indicate that the physical biases brought by the analytical model could help the parametric simulator to learn better physics in the contact-rich scenario. For instance, in the example demonstrated in Fig.~\ref{fig_abl_stapler} the ablated version fails to guide the robot hand to successfully pinch the object in the second figure. 

\noindent\textbf{Parameterized residual physics.}
To validate the necessity of introducing residual force networks to close the gap between the physics modeled in the parametric analytical simulator and that of a realistic simulator, we ablate the parametric force network and create a version named ``Ours w/o Residual Networks''. Table~\ref{tb_exp_ablations} demonstrates its role in enabling the parametric simulator to approximate realistic physics models. 



\noindent\textbf{Local residual force network.} 
To adequately leverage state and contact-related information for predicting residual contact forces, we propose to use two types of networks: 1) a local force network per contact pair residual forces and 2) a global network for additionally compensating. 
% we propose two types of networks: 1) a local force network that predicts residual contact forces between each contact pair based on the contact region information identified by the contact pair, and 2) a global residual network that predicts the residual force and torque, applied to the object's center of mass, from the global contact region. 
The local network is introduced for fine-grained approximation. We ablate this design and compare the result with our full model to validate this  (see Fig.~\ref{fig_abl_stapler} and Table~\ref{tb_exp_main}). 
% To validate this, we create an ablated version 
% % through an ablated version 
% ``Ours w/o Local Force NN'' and compare it 
% % the ablated version 
% with the full model (Fig.~\ref{fig_abl_stapler} and Table~\ref{tb_exp_main}). 
% In the example shown in Fig.~\ref{fig_abl_stapler}, ablating the local force network prevents the robot hand from establishing contacts for manipulating the object. 

%%%%%%% moved to supp %%%%%%%
% \tao{For both residual physics and residual force, people in this space are interested in their magnitude relative to the ``backbone'' physics and force. Ideally, the analytical model explains the majority of the physics and the residual one serves a minor role. I think it would be good if you happen to have such data and report whether this is indeed the case.}

\noindent\textbf{Optimizing through an analytical physics curriculum.}
We further investigate the effectiveness of the analytical curriculum design and how its design influences the result. Specifically, we create two ablated versions: 
% curriculum influence the final
% We try to ablate the current analytical physics curriculum design to validate the effectiveness of the curriculum and how
% An analytical physics curriculum is introduced
% To investigate the necessity of introduci
% physics curriculum and solving a series of easy optimization problems in each physics model and how the curriculum design would affect the performance, we create two ablated versions: 
1) ``Ours w/o Curriculum'', where the optimization starts directly from the parameterized analytical model with articulated rigid constraints imposed and the stiffest contact model, and 2) ``Ours w/ Curriculum II'', where we move some stages out from the original curriculum. 
% away from the original full path. 
Table~\ref{tb_exp_ablations}  and Fig.~\ref{fig_abl_stapler} demonstrate that both the curriculum and the optimization path will affect the model's performance. 
% As indicated by the comparisons (Table~\ref{tb_exp_ablations}  and Fig.~\ref{fig_abl_stapler}), both the curriculum and the 
% both the curriculum and the path of the optimization will affect the method's performance. Its power will be unlocked when the curriculum is carefully designed so that the previous optimized results serve as a good initialization for the following optimizations. 


% \noindent\textbf{The hybrid approach for approximating a target simulator.}
% To close the gap between the physics modeled in the model of the end of our curriculum and to optimize for a control sequence in a target simulator, we augment it using neural networks that learn to predict residual normal contact forces and residual tangential forces. To validate its effectiveness, we ablate the hybrid design, resulting in the ablated version ``Ours w/o hybrid'' and test its performance in the PyBullet simulation environment. 


% -network 
% -analytical sim base

% \noindent\textbf{Neural network design in the hybrid simulation.}
% Our design utilizes the network to predict residual contact forces from a local region with per-point contact-aware and motion-aware information. To validate such network design, we change the input information to features extracted from the point cloud capturing the contact region and create a version named ``Ours w/ Global Feat. Force NN''. We find that using the right information for predicting contact-related statistics is important both quantitatively (Table xxx) and qualitatively (Figure xxx). In the example shown in the Figure~\ref{fig_abl_stapler} where the hand utilizes two fingers to pinch the stapler and then uses the whole hand to manipulate it, 
% As shown in Figure~\ref{}, the hand fails to establish sufficient contact with the stapler and the object bounced out from the hand. 

% \noindent\textbf{Analytical sim as the base model.}



% \noindent\textbf{Curriculum optimization.}
% We design a programmable simulation engine that iteratively optimizes the robot control trajectory and performs the system identification in a curriculum of physics modeling. This way we can effectively optimize for a plausible hand trajectory in the final physics model. The final physics model with the identified parameters and the optimized hand trajectory, then serves as the starting point for further optimization. To prove the role of curriculum optimization, we ablate it and create a version ``Ours w/o curriculum''. From Table~\ref{} and Figure~\ref{}, we can observe the role of curriculum in optimizing for plausible initial hand trajectory. Ablating the previous optimization steps is hard to acquire a plausible hand trajectory. 

% \noindent\textbf{The curriculum design.}




% able -- the designs and the contacts and the tables 



% \begin{wrapfigure}[12]{r}{0pt}
% \vspace{-8ex}
% \includegraphics[width = 0.35\textwidth]{figs/abl-for-cotacts-2.pdf}
%     \caption{Effectiveness of the \textbf{hybrid physics curriculum} for robotic control optimization.}
%   % \vspace{1ex}
%   \label{fig_abl_stapler}
% \end{wrapfigure}


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.5\textwidth]{figs/abl-for-contacts-2.pdf}
%   \caption{
%   Effectiveness of the \textbf{hybrid physics curriculum} for robotic control optimization.
%   }
%   \label{fig_abl_stapler}
% \end{figure}


\begin{figure}[htbp]
  \centering
  \vspace{-20pt}
  \includegraphics[width=0.7\textwidth]{figs/abl-all.pdf}
  \vspace{-13pt}
  \caption{
  (a) Qualitative comparisons between our full method and the ablated models; (b) Training loss curve comparisons; 
  % to approximate the target simulator between our full parametric model and the version without the analytical model; 
  (c) Tracking loss curve comparisons.
  % when optimizing in the last analytical simulator between the method using full curriculum and the one using a modified version. 
  % in the last analytical
  % Effectiveness of the \textbf{hybrid physics curriculum} for robotic control optimization.
  }
  \vspace{-20pt}
  \label{fig_abl_stapler}
\end{figure}



% \begin{wraptable}[7]{r}{0.5\textwidth}
\begin{table*}[t]
    \centering
    \caption{ 
    % quantitative evaluations and comparisons to baselines % 
    \textbf{Ablation studies.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. The simulation environment is Bullet. 
    } 
	% \resizebox{\linewidth}{!}{%
    \resizebox{\textwidth}{!}{%
\begin{tabular}{@{\;}lccccc@{\;}}
        \toprule

        
        Method & \makecell[c]{$R_{\text{err}}$ ($^\circ, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  MPJPE (${mm}, \downarrow$)  & CD (${mm}, \downarrow$) & Success Rate ($\%, \uparrow$)    \\


        \cmidrule(l{0pt}r{1pt}){1-1}
        \cmidrule(l{2pt}r{2pt}){2-6}


        \makecell[l]{Ours w/o Analytical Sim.} & 44.27 & 4.39 & 29.84 & 12.91 &  0/13.73/25.49
        \\ 
        \makecell[l]{Ours w/o Residual Networks}  & 33.69 & 3.81 & \iblue{26.57} & 10.34 & 5.88/23.53/41.18
        \\ 
        \makecell[l]{Ours w/o Local Force NN} & 35.98 & 2.90 & 32.87 & 12.44 &  0/19.61/35.29
        \\ 
        \makecell[l]{Ours w/o Curriculum} & 42.40 & 4.87 & 32.61 & 13.37 &  0/17.64/29.41
        \\ 
        \makecell[l]{Ours w/ Curriculum II} & \iblue{29.58} & \iblue{2.33} & 31.61 & \iblue{10.29} &  \iblue{11.76}/\iblue{27.45}/\iblue{50.98}
        \\ 
        
        Ours & \bred{24.21} & \bred{1.97} & \bred{24.40} & \bred{9.85} & \bred{27.45}/\bred{37.25}/\bred{58.82}
        \\ 
        \bottomrule
 
    \end{tabular}
    }
    \label{tb_exp_ablations}
% \end{wraptable}
\end{table*}


==> articles/EXP-copy.tex <==


\section{Experiments} \label{sec_exp}



We conduct extensive experiments to demonstrate the effectiveness of our method. The evaluation dataset is constructed from three HOI datasets with both single-hand and bimanual manipulations (with rigid objects), with complex manipulations with non-trivial object movements, and rich and changing contacts involved (see Section~\ref{sec:exp_settings}). 
We use Shadow hand~\cite{shadowhand} and test in two simulators widely used in the embodied AI community: Bullet~\cite{coumans2016pybullet} and Isaac Gym~\cite{makoviychuk2021isaac}. 

We compare our method with both model-free approaches and model-based strategies and demonstrate the superiority of our method both quantitatively and qualitatively. We can track complex contact-rich manipulations with large object rotations, back-and-forth object movements, and changing contacts successfully in both of the two simulators, while the best-performed baseline fails (see Section~\ref{sec:retargeting_result}, Fig.~\ref{fig_res}). On average, we boost the tracking success rate by 11\%+ from the previous SOTA (see Section~\ref{sec:retargeting_result}). We make further analysis and discussions and show that the core philosophy of our work, optimizing through a quasi-physics curriculum, is potentially general and can help improve the performance of a model-free baseline (see Section~\ref{sec:exp_further_analysis}). 




\subsection{Experimental Settings} \label{sec:exp_settings}

\noindent\textbf{Datasets.} 
Our evaluation dataset is compiled from three distinct sources: the GRAB dataset~\cite{taheri2020grab}, which includes single-hand interactions with everyday objects; the TACO dataset~\cite{liu2024taco}, focusing on human manipulation of tools; and the ARCTIC dataset~\cite{fan2023arctic}, which features complex bimanual manipulations. 
For GRAB, we randomly sample a manipulation trajectory for each object. 
If its manipulation is extremely simple, we additionally sample one trajectory for it. 
The object is not considered if its corresponding manipulation is bimanual such as  \texttt{binoculars}, involves other body parts such as \texttt{bowl}, or with detailed part movements such as the \texttt{game board}. \tao{Are binoculars, bowl, and game board example names in GRAB? If so, maybe use a different font, e.g., \texttt{bowl}, to avoid confusion.}

The number of manipulation sequences from GRAB is 27. 
For TACO~\cite{liu2024taco}, we acquire data by contacting authors. 
We randomly select one sequence for each right-hand tool object. Sequences with very low quality like erroneous object motions are excluded. 14 trajectories in total are selected finally. 
For ARCTIC~\cite{fan2023arctic}, we randomly select one sequence for each object from its available manipulation trajectories, resulting in 10 sequences in total. More details are deferred to the Supp. 


\noindent\textbf{Metrics.} 
We introduce three distinct metrics to assess the quality of object tracking, the accuracy of hand tracking, and the overall success of the tracking task: %\tao{I feel that the paper overuses passive voice. It is better to keep it simple and say ``We introduce three types of metrics...''  }
1) Per-frame average object rotation error: $R_{\text{err}} = \frac{1}{N} \sum_{n=1}^N (1 - (\mathbf{q}_n \cdot \hat{\mathbf{q}}_n))$, where $\mathbf{q}_n$ is the ground-truth orientation and $\hat{\mathbf{q}}_n$ is the tracked result, represented in quaternion. 2) Per-frame average object translation error: $T_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert$, where $\mathbf{t}$ and $\mathbf{t}_n$ are ground-truth and tracked translations respectively. 3) Per-frame average hand keypoint error: $\text{MPJPE} =  \frac{1}{N} \sum_{n=1}^N  \Vert \mathbf{J}^h_n - \mathbf{J}^r_n \Vert$~\cite{qin2023anyteleop,grandia2023doc,villegas2021contact}, where $\mathbf{J}^h$ and $\mathbf{J}^r$ are keypoints for human and robot hand respectively. We manually define the keypoints and the correspondences to the human hand keypoints for the Shadow hand. 
% to the human hand 
% for the robot hand. Details are deferred to the Supp. 
4) Per-frame average hand Chamfer Distnace \tao{typo}: $\text{CD} = \frac{1}{N} \sum_{n=1}^N \text{Chamfer-Distance} (\mathbf{H}^h_n - \mathbf{H}_n )$, for evaluating whether the Shadow hand can ``densely'' track the demonstration. 5)Success rate is defined as the percentage of tracking instances deemed successful when the object's rotational error ($R_{\text{err}}$), translational error ($T_{\text{err}}$), and the Mean Per Joint Position Error in hand tracking are all below their respective predefined thresholds.  %\tao{what is this? I am less knowledgeable than an average ECCV reviewer and I don't know it. Maybe add its full name or a reference?}
Three trends of thresholds are introduced, namely  $10^\circ-10cm-10cm$, $15^\circ-15cm-15cm$, resulting in three success rates~\eric{three trends?}. \tao{yeah what are three trends?} 
% with three different  thresholds ($R_{\text{err}}-T_{\text{err}}-\text{MPJPE}$) as $10^\circ-10cm-10cm$, $15^\circ-15cm-15cm$, and $20^\circ-20cm-20cm$ respectively. 

\noindent\textbf{Baselines.}
We compare with two trends of baselines. 
For model-free approaches, since there is no prior work with exactly the same problem setting as us, we try to modify and improve a goal-driven rigid object manipulation method DGrasp~\cite{christen2022d} into two methods for tracking: 1) DGrasp-Base, where the setting is almost kept with same with the original DGrasp method. We use the first frame where the hand and the object are in contact with each other as the reference frame. Then the policy is trained to grasp the object according to the reference hand and object goal at first. After that, only the root is guided to complete the task. 2) DGrasp-Tracking, where we divide the whole sequence into several subsequences, each of which has 10 frames, and define the end frame of the subsequence as the reference frame. Then the grasping policy is used to guide the hand and gradually track the object according to the hand and the object pose of each reference frame. 
We improve the DGrasp-Tracking by optimizing the policy through the quasi-physical curriculum and create ``DGrasp-Tracking (w/ Curriculum)'' trying to improve its performance. 
% \emph{i.e.,} DGrasp-Tracking (w/ Curriculum) trying to improve its performance. 
For model-based methods, we compare with Control-VAE~\cite{yao2022controlvae} and traditional MPC approaches. 
For Control-VAE, we modify its implementation for the manipulation tracking task. We additionally consider three differentiable physics models to conduct model-predictive control for solving the task. Whether the model can approximate the target simulator decides the performance of the method.~\eric{is this claim correct? what about optimization challenges?} Taking the analytical model with the most tightened contact model 
% contact model 
% with the stiffest contact modeling
as the base model (``MPC (w/ base sim.)''), we further augment it with a general 
% model-agnostic 
smoothing strategy~\cite{suh2022bundled} and create ``MPC (w/ base sim. w/ soften)''~\eric{we should emphasize that we are comparing with state-of-the-art contact softening simulators to demonstrate the advantage of our parametrized quasi-physical simulator}. Details of baseline models are deferred to the Supp. 

\noindent\textbf{Training and evaluation settings.}
The physics curriculum is composed of three stages. In the first stage, the parameter $\alpha$ varies from 0.1 to 0.0 and the contact model stiffness is relaxed to the softest level. 
% and the contact distance threshold is kept at 0.1. 
In the second stage, $\alpha$ is fixed and the contact model stiffness varies from the softest version to the most tightened level gradually through eight stages. Details w.r.t. parameter settings are deferred to the Supp. 


In the first two stages, we alternatively optimize the trajectory $\mathcal{A}$ and parameters $\mathcal{S}$. In each optimization iteration, the $\mathcal{A}$ is optimized for 100 steps while $\mathcal{S}$ is optimized for 1000 steps. In the third stage,  $\mathcal{A}$ and $\psi$ are optimized for 256 steps in each iteration. For time-stepping, $\text{d}t$ is set to $5e-4$ in the parametric and the target simulators.

\subsection{Dexterous Manipulating Tracking}  \label{sec:retargeting_result}


We conducted thorough experiments in two widely used simulators~\cite{coumans2016pybullet,makoviychuk2021isaac}. We treat them as realistic simulated physical environments with high-fidelity and wish to track the manipulation in them. 

In summary, we can control a dexterous hand to complete a wide range of the manipulation tracking tasks with non-trivial object movements and changing contacts. As presented in Table~\ref{tb_exp_main}, we can achieve significantly higher success rates under three thresholds than the best-performed baseline in both % \tao{sounds repetitive. just say ``both''} tested simulators. Fig.~\ref{fig_res} 
further showcases qualitative examples and comparisons.  Please refer to \href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and supplementary video for animated results. 

\begin{table*}[t]
    \centering
    \caption{ 
    % quantitative evaluations and comparisons to baselines % 
    \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
    % For object rotation error ($R_{\text{err}}$), object translation error ($T_{\text{err}}$), hand average per-joint position error ($\text{MPJPE}$), and robot-MANO hand Chamfer Distance ($\text{CD}$), smaller values indicate better performance. For Success Rate, three different rates are calculated according to three groups of increasing error thresholds. 
    % Experiments are conducted on two simulators -- Bullet and Isaac Gym. 
    } 
	% \resizebox{\linewidth}{!}{%
    \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}lllccccc@{\;}}
        \toprule
        
        Simulator & ~ & Method & \makecell[c]{$R_{\text{err}}$ ($^\circ, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  MPJPE (${mm}, \downarrow$)  & CD (${mm}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
        \cmidrule(l{0pt}r{1pt}){1-3}
        \cmidrule(l{2pt}r{2pt}){4-8}

        \multirow{7}{*}{ Bullet } & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Base & 44.24 & 5.82 & 40.55 & 16.37 &  0/13.73/15.69
        \\ 
        ~ & ~ & DGrasp-Tracking & 44.45 & 5.04 & 37.56 & 14.72 &  0/15.69/15.69
        \\ 
        ~ & ~ & \makecell[l]{DGrasp-Tracking (w/ curric.)} & 33.86 & 4.60 & 30.47 & 13.53 &  7.84/\iblue{23.53}/\iblue{37.25} 
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        \cmidrule(l{1pt}r{1pt}){2-3}
        % \cmidrule(l{2pt}r{2pt}){8-12}


        ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & Control-VAE & 42.45 & \iblue{2.73} & 25.21 & 10.94 &  0/15.68/23.53
        \\ 
        ~ & ~ & MPC (w/ base sim.) & 32.56 & 3.67 & \iblue{24.62} & \iblue{10.80} & 0/15.68/31.37
        \\ 
        ~ & ~ &  \makecell[l]{MPC (w/ base sim. w/ soften)} & \iblue{31.89} & 3.63 & 28.26 & 11.31 & 0/21.57/\iblue{37.25}
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        
        \cmidrule(l{1pt}r{1pt}){2-3}
        \cmidrule(l{1pt}r{1pt}){4-8}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}

        ~ & ~ & Ours & \bred{24.21} & \bred{1.97} & \bred{24.40} & \bred{9.85} & \bred{27.45}/\bred{37.25}/\bred{58.82}
        \\ 
        
        \cmidrule(l{1pt}r{1pt}){1-3}
        \cmidrule(l{1pt}r{1pt}){4-8}


        \multirow{7}{*}{ Isaac Gym } & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Base & 36.41 & 4.56 & 50.97 & 18.78 & 0/7.84 /7.84 
        \\ 
        ~ & ~ & DGrasp-Tracking & 44.71 & 5.57 & 41.53 & 16.72 & 0/0/7.84 
        \\ 
        ~ & ~ & \makecell[l]{DGrasp-Tracking (w/ curric,)} & 38.75 & 5.13 & 40.09 & 16.26 & 0/\iblue{23.53}/\iblue{31.37} 
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        \cmidrule(l{1pt}r{1pt}){2-3}
        % \cmidrule(l{2pt}r{2pt}){8-12}


        ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Based} } & Control-VAE & \iblue{35.40} & 4.61 & 27.63 & 13.17 & 0/13.73/29.41
        \\ 
        ~ & ~ & MPC (w/ base sim.) & 37.23 & 4.73 & \bred{23.19} & \bred{9.75} & 0/15.69/\iblue{31.37}
        \\ 
        ~ & ~ &  \makecell[l]{MPC (w/ base sim. w/ soften)} & 36.40 & \iblue{4.46} & \iblue{23.27} & 10.34 & 0/9.80/23.53
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        
        \cmidrule(l{1pt}r{1pt}){2-3}
        \cmidrule(l{1pt}r{1pt}){4-8}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}

        ~ & ~ & Ours & \bred{25.97} & \bred{2.08} & {25.33} & \iblue{10.31} & \bred{21.57}/\bred{43.14}/\bred{56.86}
        \\ 

        \bottomrule
 
    \end{tabular}
    }
    \label{tb_exp_main}
\end{table*} 



\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figs/all-res-8.pdf}
  \vspace{-20pt}
  \caption{
  \textbf{Qualitative comparisons. }
  % on the \textbf{GRAB, GRAB (Beta), HOI4D, and ARCTIC} test sets. 
  Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_res}
  \vspace{-20pt}
\end{figure}


\begin{figure}[htbp]
\vspace{-20pt}
  \centering
  \includegraphics[width=\textwidth]{figs/rl-curriculum.pdf}
  % \vspace{-20pt}
  \caption{
  Visual evidence on boosting DGrasp-Tracking's performance via optimizing it through a physics curriculum. 
  % Effectiveness of the optimization homotopy with the quasi-physics curriculum on helping reinforcement learning to find better policies. 
  % Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_rl_curriculum}
  \vspace{-16pt}
\end{figure}




% \subsection{} \label{sec:retargeting_result}

% \todo{more analysis on the experiments such as the training curves and recovery actions}


% \todo{analysis on the curriculum optimization path }

% \todo{analysis on the gap between the final sim and a target sim}


% \noindent\textbf{Manipulating daily objects.} 
% We can drive the dexterous hand to complete a wide range of tracking tasks such as large object re-orientations, back-and-force object movements, and changing contacts. However, compared to our effectiveness, the improved RL baseline for tracking fails to solve the corresponding tracking problem. 
% \todo{details for each subfigure}


\noindent\textbf{Complex manipulations.} 
For examples shown in Fig.~\ref{fig_res}, we can complete the tracking task on examples with large object re-orientations and complicated tool-using (\textit{Fig. (a,b,c)}). However, DGrasp-Tracking fails to establish sufficient contact for correct manipulating the object. In more detail, in Fig.~\ref{fig_res}(b), the bunny gradually bounced out from the hand in Bullet, while our method does not suffer from this difficulty. In Fig.~\ref{fig_res}(c), the spoon can be successfully picked up and waved back-and-force in our method， while DGrasp-Tracking loses the track in the very beginning. 


\noindent\textbf{Bimanual manipulations.}   
% We are able to track the bimanual manipulations as well. In the example shown in Fig.~\ref{}, our object tracking result is similar to the reference. However, the DGrasp-Tracking baseline model cannot give good object-tracking results. 
 We are able to track the bimanual manipulations as well. As the example shown in Fig.~\ref{fig_res}(d) where two hands cooperate with each other to relocate the object, DGrasp-Tracking cannot track the object accurately. But ours is obviously much better. 
 % For instance, in the example shown in Fig.~\ref{fig_res}, ours object trajectory is closer to the reference than that yielded by DGrasp-Tracking.
 
 % In the example shown in Fig.~\ref{fig_res}, our object tracking result is close to the reference. However, the DGrasp-Tracking model cannot yield good object-tracking results. 


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=\textwidth]{figs/rl-curriculum.pdf}
%   % \vspace{-20pt}
%   \caption{
%   Effectiveness of the optimization homotopy with the quasi-physics curriculum on helping reinforcement learning to find better policies. Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
%   }
%   \label{fig_rl_curriculum}
%   % \vspace{-16pt}
% \end{figure}



\subsection{Further Analysis and Discussions} \label{sec:exp_further_analysis}

\noindent\textbf{Could model-free methods benefit from the physics curriculum?}
% the homotopy optimization through the physics curriculum help with improving RL-based methods?} 
% It is a natural question to ask whether the physics curriculum, if aims at softening physics and creating a path of simulated environment to aid the difficulty of the optimization in the scenario of contact-rich manipulation, would be a general approach and also works for model-free strategies. We investigate this point and demonstrate its potential to guide RL algorithms to find better policies to complete the task. As demonstrated quantitatively in Table~\ref{tb_exp_main} and comparisons shown in Fig.~\ref{fig_rl_curriculum}. 
% \todo{more analysis here}
Beyond the demonstrated merits of our quasi-physical simulators, we further investigate whether model-free strategies can benefit from it. We create the ``DGrasp-Tracking (w/ Curriculum)'' and compare its performance with the original DGrasp-Tracking model. As presented in Table~\ref{tb_exp_main} and the visual comparisons shown in Fig.~\ref{fig_rl_curriculum}, DGrasp-Tracking can indeed benefit from a well-designed physics curriculum. As examples presented in Fig.~\ref{fig_rl_curriculum}, the curriculum can help it almost complete difficult tracking tasks where the original version suffers a lot. 
% shows us qualitative evidence of its effectiveness. Solving the difficult optimization problem involving complex and tough dynamics via optimizing through a well-designed physics curriculum is a potentially general approach where various methods' performance can be boosted. 



\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figs/mpc_robustness.pdf}
  % \vspace{-20pt}
  \caption{
  \textbf{Robustness of MPC. } MPC tries to track the object even after experiencing a dangerous period with the tendency to lose track. While the trajectory yielded by open-loop optimization fails. 
  % Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_mpc_robustness}
  % \vspace{-16pt}
\end{figure}


\noindent\textbf{Robustness of MPC.} 
Fig.~\ref{fig_mpc_robustness} shows an example demonstrating tracking robustness. In this challenging example where rich contacts between fingers and the palm with the mouse are frequently established and broken, the control sequence optimized in an open-loop manner struggles with keep contacting the mouse, and the tracking is lost finally. However, with the optimized model, the trajectories produced by MPC can successfully maintain enough contact with the object and track the sequence naturally.~\eric{I am not sure what we want to deliver here? MPC is better than open loop trajectory optimization? What does it do with our method?}    


















































We conduct extensive experiments to demonstrate the effectiveness of our method. The evaluation dataset is constructed from three HOI datasets with both single-hand and bimanual manipulations (with rigid objects), with complex manipulations with non-trivial object movements, and rich and changing contacts involved (see Section~\ref{sec:exp_settings}). 
% namely GRAB~\cite{taheri2020grab}, containing single-hand interactions with daily objects, TACO~\cite{liu2024taco}, containing humans manipulating tools, and ARCTIC~\cite{fan2023arctic} with bimanual manipulations (see Section~\ref{sec:exp_settings}). 
We use Shadow hand~\cite{shadowhand} and test in two simulators widely used in the embodied AI community: Bullet~\cite{coumans2016pybullet} and Isaac Gym~\cite{makoviychuk2021isaac}. 
% We use our method to control a Shadow hand~\cite{shadowhand} to perform similar manipulations in two simulation environments widely used in robotics: Bullet~\cite{coumans2016pybullet} and Isaac Gym~\cite{makoviychuk2021isaac}. 
We compare our method with both model-free approaches and model-based strategies and demonstrate the superiority of our method both quantitatively and qualitatively. We can track complex contact-rich manipulations with large object rotations, back-and-forth object movements, and changing contacts successfully in both of the two simulators, while the best-performed baseline fails (see Section~\ref{sec:retargeting_result}, Fig.~\ref{fig_res}). On average, we boost the tracking success rate by 11\%+ from the previous SOTA (see Section~\ref{sec:retargeting_result}). We make further analysis and discussions and show that the core philosophy of our work, optimizing through a quasi-physics curriculum, is potentially general and can help improve the performance of a model-free baseline (see Section~\ref{sec:exp_further_analysis}). 

% to perform human-like manipulations in both of the two tested simulation environment, 

% describing how humans manipulate various kinds of rigid objects 
% a dataset describing how humans manipulate objects 
% We train all models on the same training dataset and introduce four four test sets with different levels of domain shift to assess their denoising ability and the generalization ability (see Section~\ref{sec_gene_denoising}). Moreover, we demonstrate the ability of our denoising method to produce multiple reasonable solutions for a single input in Section~\ref{sec_stochastic_denoising}. At last, we show various applications that we can support (Section~\ref{sec:applications}). 
% \textit{Another series of experiments using a different training set} is presented in the Appendix~\ref{sec_appen_hoi_denoising_exp}.


\subsection{Experimental Settings} \label{sec:exp_settings}

\noindent\textbf{Datasets.} 
This revision aims to enhance clarity and formality in describing the dataset selection process for the evaluation. Our evaluation dataset is compiled from three distinct sources: the GRAB dataset~\cite{taheri2020grab}, which includes single-hand interactions with everyday objects; the TACO dataset~\cite{liu2024taco}, focusing on human manipulation of tools; and the ARCTIC dataset~\cite{fan2023arctic}, which features complex bimanual manipulations. For the GRAB dataset, we randomly sample a manipulation trajectory for each object. If its manipulation is relatively simple like simple grasping, we additionally sample one trajectory for it. The object is not considered if the manipulation is bimanual such as binoculars, or requires interaction with other body parts like the mouse such as the bowl, or the manipulation involves detailed part movements such as the game board, or the manipulation is not conducted supported on a table such as handle. The total manipulation sequences selected from GRAB is 27. 
For TACO~\cite{liu2024taco}, we randomly select one sequence for each right-hand tool object. Sequences with very low quality like totally wrong trajectories are excluded. 14 trajectories in total are selected finally. 
For ARCTIC~\cite{fan2023arctic}, we randomly select one sequence for each object from its available manipulation trajectories, resulting in 10 sequences in total. More details are deferred to the Supp. 
% Objects are not considered if their manipulations are bimanual such as binoculars,


\noindent\textbf{Metrics.} 
We introduce three distinct metrics to assess the quality of object tracking, the accuracy of hand tracking, and the overall success of the tracking task: 1) Per-frame average object rotation error: $R_{\text{err}} = \frac{1}{N} \sum_{n=1}^N (1 - (\mathbf{q}_n \cdot \hat{\mathbf{q}}_n))$, where $\mathbf{q}_n$ is the GT orientation and $\hat{\mathbf{q}}_n$ is the tracked result, represented in quaternion. 2) Per-frame average object translation error: $T_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert$, where $\mathbf{t}$ and $\mathbf{t}_n$ are GT and tracked translations respectively. 3) Per-frame average hand keypoint error: $\text{MPJPE} =  \frac{1}{N} \sum_{n=1}^N  \Vert \mathbf{J}^h_n - \mathbf{J}^r_n \Vert$~\cite{qin2023anyteleop,grandia2023doc,villegas2021contact}, where $\mathbf{J}^h$ and $\mathbf{J}^r$ are keypoints for human and robot hand respectively. We manually define the keypoints and the correspondences to the human hand for the robot hand. Details are deferred to the Supp. 4) Per-frame average hand Chamfer Distnace: $\text{CD} = \frac{1}{N} \sum_{n=1}^N \text{Chamfer-Distance} (\mathbf{H}^h_n - \mathbf{H}_n )$, for evaluating whether the robot hand can ``densely'' track the demonstration. 5) Sucess rate with threshold ($R_{\text{err}}-T_{\text{err}}-\text{MPJPE}$) $10^\circ-10cm-10cm$, $15^\circ-15cm-15cm$, and $20^\circ-20cm-20cm$ respectively. 

\noindent\textbf{Baselines.}
Our comparative analysis encompasses two primary categories of baseline methodologies.
In the realm of model-free approaches, due to the absence of prior work mirroring our exact problem configuration, we adapt and enhance the goal-driven rigid object manipulation method known as DGrasp~\cite{christen2022d}. This adaptation materializes into two distinct tracking methodologies: 1) DGrasp-Base, where the setting is almost kept with same with the original DGrasp method. We use the first frame where the hand and the object are in contact with each other as the reference frame. Then the policy is trained to grasp the object according to the reference hand and object goal at first. After that, only the root is guided to complete the task. 2) DGrasp-Tracking, where we divide the whole sequence into several subsequences, each of which has 10 frames, and define the end frame of the subsequence as the reference frame. Then the grasping policy is used to guide the hand and gradually track the object according to the hand and the object pose of each reference frame. 
We improve the DGrasp-Tracking by optimizing the policy through the quasi-physical curriculum, \emph{i.e.,} DGrasp-Tracking (w/ Curriculum) trying to improve its performance. 
For model-based methods, we compare with Control-VAE~\cite{yao2022controlvae} and traditional MPC approaches. 
For Control-VAE, we modify its implementation for the manipulation tracking task. We additionally consider three differentiable physics models to conduct model-predictive control for solving the task. Whether the model can approximate the target simulator decides the performance of the method. Taking the analytical model with the stiffest contact modeling as the base model (``MPC (w/ base sim.)''), we further augment it with a model-agnostic smoothing strategy~\cite{suh2022bundled} and create ``MPC (w/ base sim. w/ soften)''. Details of baseline models are deferred to the Supp. 

\noindent\textbf{Training and evaluation settings.}
The physics curriculum is composed of three stages. In the first stage, the parameter $\alpha$ varies from 0.1 to 0.0 and the contact model stiffness is relaxed to the softest level. 
% and the contact distance threshold is kept at 0.1. 
In the second stage, $\alpha$ is fixed and the contact model stiffness varies from the softest version to the most tightened level gradually through eight stages. Details w.r.t. parameter settings are deferred to the Supp. 
% and eight stages 
% and the contact distance threshold parameter $d^c$ varies from 0.1 to 0.0, resulting in 8 stages gradually. 
% is set to $0.1,0.05,0.03,0.025,0.02,0.015,0.01,0$ gradually. 
% The residual force networks are not activated and always output zero values. In the third stage, the residual networks are activated and optimized to approximate the behavior of a target simulator.
In the first two stages, we alternatively optimize the trajectory $\mathcal{A}$ and parameters $\mathcal{S}$. In each optimization iteration, the $\mathcal{A}$ is optimized for 100 steps while $\mathcal{S}$ is optimized for 1000 steps. In the third stage,  $\mathcal{A}$ and $\psi$ are optimized for 256 steps in each iteration. For time-stepping, $\text{d}t$ is set to $5e-4$ in the parametric and the target simulators. The articulated multi-body is controlled by joint motors and root velocities in the parametric simulator while PD control~\cite{tan2012advances}  is leveraged in the target simulators. 
% More details are deferred to the Supp. 

\subsection{Dexterous Manipulating Tracking}  \label{sec:retargeting_result}


We conducted thorough experiments in two widely used simulators~\cite{coumans2016pybullet,makoviychuk2021isaac}. We treat them as realistic simulated physical environments with high-fidelity and wish to track the manipulation in them. 
% as realistic physical models and wish to physically track the manipulation in them. 
The quantitative results are summarized in Table~\ref{tb_exp_main}. And the qualitative comparisons are presented in Figure~\ref{fig_res}. Please refer to \href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and supplementary video for animated results. 
In summary, we can control a dexterous hand to complete a wide range of the manipulation tracking tasks with non-trivial object movements and changing contacts. As presented in Table~\ref{tb_exp_main}, we can achieve significantly higher success rates under three thresholds than the best-performed j 
% As shown in Table~\ref{tb_exp_main}, our method can achieve obviously better performance than baseline models. 
% Our evaluation demonstrates that we can bypass the best-performed baseline by a large margin regarding the overall task completion in both Bullet~\cite{coumans2016pybullet} and Isaac Gym~\cite{makoviychuk2021isaac}. 


\begin{table*}[t]
    \centering
    \caption{ 
    % quantitative evaluations and comparisons to baselines % 
    \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
    % For object rotation error ($R_{\text{err}}$), object translation error ($T_{\text{err}}$), hand average per-joint position error ($\text{MPJPE}$), and robot-MANO hand Chamfer Distance ($\text{CD}$), smaller values indicate better performance. For Success Rate, three different rates are calculated according to three groups of increasing error thresholds. 
    % Experiments are conducted on two simulators -- Bullet and Isaac Gym. 
    } 
	% \resizebox{\linewidth}{!}{%
    \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}lllccccc@{\;}}
        \toprule
        
        Simulator & ~ & Method & \makecell[c]{$R_{\text{err}}$ ($^\circ, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  MPJPE (${mm}, \downarrow$)  & CD (${mm}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
        \cmidrule(l{0pt}r{1pt}){1-3}
        \cmidrule(l{2pt}r{2pt}){4-8}

        \multirow{7}{*}{ Bullet } & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Base & 44.24 & 5.82 & 40.55 & 16.37 &  0/13.73/15.69
        \\ 
        ~ & ~ & DGrasp-Tracking & 44.45 & 5.04 & 37.56 & 14.72 &  0/15.69/15.69
        \\ 
        ~ & ~ & \makecell[l]{DGrasp-Tracking (w/ curric.)} & 33.86 & 4.60 & 30.47 & 13.53 &  7.84/\iblue{23.53}/\iblue{37.25} 
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        \cmidrule(l{1pt}r{1pt}){2-3}
        % \cmidrule(l{2pt}r{2pt}){8-12}


        ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & Control-VAE & 42.45 & \iblue{2.73} & 25.21 & 10.94 &  0/15.68/23.53
        \\ 
        ~ & ~ & MPC (w/ base sim.) & 32.56 & 3.67 & \iblue{24.62} & \iblue{10.80} & 0/15.68/31.37
        \\ 
        ~ & ~ &  \makecell[l]{MPC (w/ base sim. w/ soften)} & \iblue{31.89} & 3.63 & 28.26 & 11.31 & 0/21.57/\iblue{37.25}
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        
        \cmidrule(l{1pt}r{1pt}){2-3}
        \cmidrule(l{1pt}r{1pt}){4-8}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}

        ~ & ~ & Ours & \bred{24.21} & \bred{1.97} & \bred{24.40} & \bred{9.85} & \bred{27.45}/\bred{37.25}/\bred{58.82}
        \\ 
        
        \cmidrule(l{1pt}r{1pt}){1-3}
        \cmidrule(l{1pt}r{1pt}){4-8}


        \multirow{7}{*}{ Isaac Gym } & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Base & 36.41 & 4.56 & 50.97 & 18.78 & 0/7.84 /7.84 
        \\ 
        ~ & ~ & DGrasp-Tracking & 44.71 & 5.57 & 41.53 & 16.72 & 0/0/7.84 
        \\ 
        ~ & ~ & \makecell[l]{DGrasp-Tracking (w/ curric,)} & 38.75 & 5.13 & 40.09 & 16.26 & 0/\iblue{23.53}/\iblue{31.37} 
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        \cmidrule(l{1pt}r{1pt}){2-3}
        % \cmidrule(l{2pt}r{2pt}){8-12}


        ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Based} } & Control-VAE & \iblue{35.40} & 4.61 & 27.63 & 13.17 & 0/13.73/29.41
        \\ 
        ~ & ~ & MPC (w/ base sim.) & 37.23 & 4.73 & \bred{23.19} & \bred{9.75} & 0/15.69/\iblue{31.37}
        \\ 
        ~ & ~ &  \makecell[l]{MPC (w/ base sim. w/ soften)} & 36.40 & \iblue{4.46} & \iblue{23.27} & 10.34 & 0/9.80/23.53
        \\ 
        % \cmidrule(l{15pt}r{17pt}){3-9}
        
        \cmidrule(l{1pt}r{1pt}){2-3}
        \cmidrule(l{1pt}r{1pt}){4-8}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}

        ~ & ~ & Ours & \bred{25.97} & \bred{2.08} & {25.33} & \iblue{10.31} & \bred{21.57}/\bred{43.14}/\bred{56.86}
        \\ 

        \bottomrule
 
    \end{tabular}
    }
    \label{tb_exp_main}
\end{table*} 



\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figs/all-res-7.pdf}
  \vspace{-20pt}
  \caption{
  \textbf{Qualitative comparisons. }
  % on the \textbf{GRAB, GRAB (Beta), HOI4D, and ARCTIC} test sets. 
  Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_res}
  \vspace{-20pt}
\end{figure}


\begin{figure}[htbp]
\vspace{-20pt}
  \centering
  \includegraphics[width=\textwidth]{figs/rl-curriculum.pdf}
  % \vspace{-20pt}
  \caption{
  Visual evidence on boosting DGrasp-Tracking's performance via optimizing it through a physics curriculum. 
  % Effectiveness of the optimization homotopy with the quasi-physics curriculum on helping reinforcement learning to find better policies. 
  % Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_rl_curriculum}
  \vspace{-16pt}
\end{figure}




% \subsection{} \label{sec:retargeting_result}

% \todo{more analysis on the experiments such as the training curves and recovery actions}


% \todo{analysis on the curriculum optimization path }

% \todo{analysis on the gap between the final sim and a target sim}


% \noindent\textbf{Manipulating daily objects.} 
% We can drive the dexterous hand to complete a wide range of tracking tasks such as large object re-orientations, back-and-force object movements, and changing contacts. However, compared to our effectiveness, the improved RL baseline for tracking fails to solve the corresponding tracking problem. 
% \todo{details for each subfigure}


\noindent\textbf{Complex manipulations.} 



\noindent\textbf{Bimanual manipulations.}   
% We are able to track the bimanual manipulations as well. In the example shown in Fig.~\ref{}, our object tracking result is similar to the reference. However, the DGrasp-Tracking baseline model cannot give good object-tracking results. 
 We are able to track the bimanual manipulations as well. For instance, in the example shown in Fig.~\ref{fig_res}, ours object trajectory is closer to the reference than that yielded by DGrasp-Tracking.
 % In the example shown in Fig.~\ref{fig_res}, our object tracking result is close to the reference. However, the DGrasp-Tracking model cannot yield good object-tracking results. 


% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=\textwidth]{figs/rl-curriculum.pdf}
%   % \vspace{-20pt}
%   \caption{
%   Effectiveness of the optimization homotopy with the quasi-physics curriculum on helping reinforcement learning to find better policies. Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
%   }
%   \label{fig_rl_curriculum}
%   % \vspace{-16pt}
% \end{figure}



\subsection{Further Analysis and Discussions} \label{sec:exp_further_analysis}

\noindent\textbf{Could model-free methods benefit from the physics curriculum?}
% the homotopy optimization through the physics curriculum help with improving RL-based methods?} 
% It is a natural question to ask whether the physics curriculum, if aims at softening physics and creating a path of simulated environment to aid the difficulty of the optimization in the scenario of contact-rich manipulation, would be a general approach and also works for model-free strategies. We investigate this point and demonstrate its potential to guide RL algorithms to find better policies to complete the task. As demonstrated quantitatively in Table~\ref{tb_exp_main} and comparisons shown in Fig.~\ref{fig_rl_curriculum}. 
% \todo{more analysis here}
Beyond the demonstrated merits of our quasi-physical simulators, we further investigate whether model-free strategies can benefit from it. We create the ``DGrasp-Tracking (w/ Curriculum)'' and compare its performance with the original DGrasp-Tracking model. As presented in Table~\ref{tb_exp_main} and the visual comparisons shown in Fig.~\ref{fig_rl_curriculum}, DGrasp-Tracking can indeed benefit from a well-designed physics curriculum. As examples presented in Fig.~\ref{fig_rl_curriculum}, the curriculum can help it almost complete difficult tracking tasks where the original version suffers a lot. 
% shows us qualitative evidence of its effectiveness. Solving the difficult optimization problem involving complex and tough dynamics via optimizing through a well-designed physics curriculum is a potentially general approach where various methods' performance can be boosted. 



\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figs/mpc_robustness.pdf}
  % \vspace{-20pt}
  \caption{
  \textbf{Robustness of MPC. } MPC tries to track the object even after experiencing a dangerous period with the tendency to lose track. While the trajectory yielded by open-loop optimization fails. 
  % Please refer to \textbf{\href{https://quasi-physical-sims.github.io/quasi-physical-sims-for-dex-manip/}{our website} and {the supplementary video} } for animated results.
  }
  \label{fig_mpc_robustness}
  % \vspace{-16pt}
\end{figure}


\noindent\textbf{Robustness of MPC.} 
Fig.~\ref{fig_mpc_robustness} shows an example demonstrating tracking robustness. In this challenging example where rich contacts between fingers and the palm with the mouse are frequently established and broken, the control sequence optimized in an open-loop manner struggles with keep contacting the mouse, and the tracking is lost finally. However, with the optimized model, the trajectories produced by MPC can successfully maintain enough contact with the object and track the sequence naturally.    



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

